Scaling Polyhedral Neural Network Verification on GPUs

Certifying the robustness of neural networks against adversarial attacks is essential to their reliable adoption in safety-critical systems such as autonomous driving and medical diagnosis. Unfortunately, state-of-the-art verifiers either do not scale to bigger networks or are too imprecise to prove robustness, limiting their practical adoption. In this work, we introduce GPUPoly, a scalable verifier that can prove the robustness of significantly larger deep neural networks than previously possible. The key technical insight behind GPUPoly is the design of custom, sound polyhedra algorithms for neural network verification on a GPU. Our algorithms leverage the available GPU parallelism and inherent sparsity of the underlying verification task. GPUPoly scales to large networks: for example, it can prove the robustness of a 1M neuron, 34-layer deep residual network in approximately 34.5 ms. We believe GPUPoly is a promising step towards practical verification of real-world neural networks.

==> abstract.tex <==
\begin{abstract}
Certifying the robustness of neural networks against adversarial attacks is critical to their reliable adoption in real-world systems including autonomous driving and medical diagnosis. Unfortunately, state-of-the-art verifiers either do not scale to larger networks or are too imprecise to prove robustness, which limits their practical adoption.
In this work, we introduce \tool, a scalable verifier that can prove the robustness of significantly larger deep neural networks than previously possible. The key insight behind \tool is the design of custom, sound polyhedra algorithms for neural network verification on a GPU. Our algorithms leverage the available GPU parallelism and inherent sparsity of the underlying neural network verification task.
\tool scales to very large networks: for example, it can prove the robustness of a 1M neuron, 34-layer deep residual network in about 1 minute. We believe \tool is a promising step towards the practical verification of large real-world networks.
\end{abstract} 

==> networks.tex <==
\begin{figure*}[h!t]
\centering
\begin{tikzpicture}[scale=0.9]
\tikzstyle{style2}[black]=[draw=#1,fill=none,opacity=1.0,line width=1,->]
%\begin{equation*}
%\begin{aligned}
%\text{Input} \rightarrow \text{Affine} \rightarrow \text{ReLU} \rightarrow \text{Affine} \rightarrow \text{ReLU} \rightarrow \text{Affine} \rightarrow \text{Output}
%\end{aligned}
%\end{equation*}
\begin{scope}
\coordinate (p1) at (-1, 0) ;
\coordinate (p2) at (1.2, 0) ;
\coordinate (p3) at (3, 0) ;
\coordinate (p4) at (5.2, 0) ;
\coordinate (p5) at (7, 0) ;
\coordinate (p6) at (9.2, 0) ;
\coordinate (p7) at (11, 0) ;
\coordinate (origin) at (0, 0) ;
\filldraw[style2] (0,0) -- (1,0);
\filldraw[style2] (2,0) -- (3,0);
\filldraw[style2] (4.2,0) -- (5,0);
\filldraw[style2] (6,0) -- (7,0);
\filldraw[style2] (8.2,0) -- (9.2,0);
\filldraw[style2] (10,0) -- (11,0);
%\filldraw[style2] (12,0) -- (13,0);

		\fill[black,font=\small]
			(p1) node [right] {Input$^1$}
			(p2) node [right] {FC$^2$}
			(p3) node [right] {ReLU$^3$}
			(p4) node [right] {FC$^4$}
			(p5) node [right] {ReLU$^5$}
			(p6) node [right] {FC$^6$}
			(p7) node [right] {Output$^7$};
			%(6,-0.5) node [below] {(a) Fully connected network};
\end{scope}

\begin{scope}
\coordinate (p1) at (-1, -0.75) ;
\coordinate (p2) at (1, -0.75) ;
\coordinate (p3) at (3, -0.75) ;
\coordinate (p4) at (5, -0.75) ;
\coordinate (p5) at (7, -0.75) ;
\coordinate (p6) at (9.2, -0.75) ;
\coordinate (p7) at (11, -0.75) ;
\filldraw[style2] (0.1,-0.75) -- (1,-0.75);
\filldraw[style2] (2.1,-0.75) -- (3,-0.75);
\filldraw[style2] (4.2,-0.75) -- (5,-0.75);
\filldraw[style2] (6.1,-0.75) -- (7,-0.75);
\filldraw[style2] (8.2,-0.75) -- (9.2,-0.75);
\filldraw[style2] (10,-0.75) -- (11,-0.75);
%\filldraw[style2] (12,0) -- (13,0);

		\fill[black,font=\small]
			(p1) node [right] {Input$^1$}
			(p2) node [right] {Conv$^2$}
			(p3) node [right] {ReLU$^3$}
			(p4) node [right] {Conv$^4$}
			(p5) node [right] {ReLU$^5$}
			(p6) node [right] {FC$^6$}
			(p7) node [right] {Output$^7$};
			%(6,-2) node [below] {(b) Convolutional network};

\end{scope}

\begin{scope}
\coordinate (p1) at (-1, -2) ;
\coordinate (p2) at (1, -2) ;
\coordinate (p3) at (3, -2) ;
\coordinate (p4) at (5, -1.5) ;
\coordinate (p8) at (5, -2.5) ;
\coordinate (p5) at (7, -2) ;
\coordinate (p6) at (9.2, -2) ;
\coordinate (p7) at (11.3, -2) ;
\coordinate (p9) at (13.5, -2) ;
\coordinate (p10) at (15.5, -2) ;
\coordinate (p11) at (7, -1.5) ;

\filldraw[style2] (0.1,-2) -- (1,-2);
\filldraw[style2] (2.1,-2) -- (3,-2);
\filldraw[style2] (4.2,-2) -- (5,-1.5);
\filldraw[style2] (6.1,-1.5) -- (7,-2);
\filldraw[style2] (4.2,-2) -- (5,-2.5);
\filldraw[style2] (6.1,-2.5) -- (7,-2);
\filldraw[style2] (8.2,-2) -- (9.2,-2);
\filldraw[style2] (10.4,-2) -- (11.3,-2);
\filldraw[style2] (12.6,-2) -- (13.5,-2);
\filldraw[style2] (14.5,-2) -- (15.5,-2);

		\fill[black,font=\small]
			(p1) node [right] {Input$^1$}
			(p2) node [right] {Conv$^2$}
			(p3) node [right] {ReLU$^3$}
			(p4) node [right] {Conv$^4$}
			(p8) node [right] {Conv$^5$}
            (p5) node [right] {ReLU$^6$}
            (p6) node [right] {Conv$^7$}
			(p7) node [right] {ReLU$^8$}
			(p9) node [right] {FC$^9$}
            (p10) node [right] {Output$^{10}$};
			%(6,-4.5) node [below] {(c) Residual network};
\end{scope}


\end{tikzpicture}

\caption{Sketches of considered neural network architectures. }
\label{Fi:networks}
%\vspace{-5mm}
\end{figure*}


==> neural_network.tex <==
\begin{figure*}[h!t]

\centering
\begin{tikzpicture}[font=\tiny\sffamily][scale=1]
    \node[shape=circle,draw=black] (A) at (0,0) {$x_{1}^{0}$};
    \node[shape=circle,draw=black] (B) at (0,-1.5) {$x_{2}^{0}$};
    \node[shape=circle,draw=green] (C) at (2.5,0) {$x_{1}^{1}$};
    \node[shape=circle,draw=green] (D) at (2.5,-1.5) {$x_{2}^{1}$};
    \node[shape=circle,draw=red] (E) at (5,0) {$x_{1}^{2}$};
    \node[shape=circle,draw=red] (F) at (5,-1.5) {$x_{2}^{2}$};
    \node[shape=circle,draw=green] (G) at (7.5,0) {$x_{1}^{3}$} ;
    \node[shape=circle,draw=green] (H) at (7.5,-1.5) {$x_{2}^{3}$} ;
     \node[shape=circle,draw=red] (I) at (10,0) {$x_{1}^{4}$} ;
    \node[shape=circle,draw=red] (J) at (10,-1.5) {$x_{2}^{4}$} ;
    \node[shape=circle,draw=green] (K) at (12.5,0) {$x_{1}^{5}$} ;
    \node[shape=circle,draw=green] (L) at (12.5,-1.5) {$x_{2}^{5}$} ;
    \node[shape=circle,draw=blue] (M) at (15,0) {$x_{1}^{6}$} ;
    \node[shape=circle,draw=blue] (N) at (15,-1.5) {$x_{2}^{6}$} ;

    \path [->] (A) edge node[left,above] {1} (C);
    \path [->](B) edge node[left,below] {-1} (D);
    \path [->](A) edge node[pos=0.25,left,above] {1} (D);
    \path [->](B) edge node[pos=0.25,left,above] {1} (C);
    
    \path [->](C) edge node[left,above] {$\max(0,x_{1}^{1})$} (E);
    \path [->](D) edge node[left,below] {$\max(0,x_{2}^{1})$} (F);
    
    \path [->] (E) edge node[left,above] {1} (G);
    \path [->](F) edge node[left,below] {-1} (H);
    \path [->](E) edge node[pos=0.25,left,above] {1} (H);
    \path [->](F) edge node[pos=0.25,left,above] {1} (G);
    \path [->](G) edge node[left,above] {$\max(0,x_{1}^{3})$} (I);
    \path [->](H) edge node[left,below] {$\max(0,x_{2}^{3})$} (J);
    \path [->] (-1,0) edge node[left,above] {} (A);
    \path [->](-1,-1.5) edge node[left,below] {} (B);
    \path [->] (I) edge node[left,above] {1} (K);
    \path [->](J) edge node[pos=0.25,left,above] {1} (K);
    \path [->] (I) edge node[pos=0.25,left,above] {0} (L);
    \path [->](J) edge node[left,below] {1} (L);

    \path [->] (K) edge node[left,above] {+1.2} (M);
    \path [->](L) edge node[left,below] {+0} (N);


    \coordinate (x1) at (A);
\node at (x1) [above=2.6mm  of x1] {[0,0.5]};





\coordinate (x2) at (B);
\node at (x2) [above=2.6mm  of x2] {[0,0.5]};


 \coordinate (x3) at (C);
 \node at (x3) [above=2.6mm  of x3,blue] {[0,1]};
\node at (x3) [above=5.5mm  of x3] { $\begin{aligned}
x_{1}^{1}\leq &x_{1}^{1} \leq x_{1}^{1}\\
x_{1}^{0} +x_{2}^{0}\leq &x_{1}^{1} \leq x_{1}^{0}+x_{2}^{0}\\
0\leq &x_{1}^{1} \leq 1\\
\end{aligned}$ };


\coordinate (x4) at (D);
 \node at (x4) [above=2.6mm  of x4,blue] {[-0.5,0.5]};
\node at (x4) [below=5.5mm  of x4] { $\begin{aligned}
x_{2}^{1}\leq &x_{2}^{1} \leq x_{2}^{1}\\
x_{1}^{0} -x_{2}^{0}\leq &x_{2}^{1} \leq x_{1}^{0}-x_{2}^{0}\\
-0.5\leq &x_{2}^{1} \leq 0.5\\
\end{aligned}$ };



\coordinate (x5) at (E);
 \node at (x5) [above=2.6mm  of x5,blue] {[0,1]};
\node at (x5) [above=5.5mm  of x5,gray] { $x_{1}^{1}\leq x_{1}^{2} \leq x_{1}^{1}$ };

\coordinate (x6) at (F);
 \node at (x6) [above=2.6mm  of x6,blue] {[0,0.5]};
\node at (x6) [below=5.5mm  of x6,gray] { $0\leq x_{2}^{2} \leq 0.5x_{2}^{1}+0.25$ };
\coordinate (x7) at (G);
 \node at (x7) [above=2.6mm  of x7,blue] {[0,1.5]};
\node at (x7) [above=5.5mm  of x7] { $\begin{aligned}
x_{1}^{3}\leq &x_{1}^{3} \leq x_{1}^{3}\\
x_{1}^{2} +x_{2}^{2}\leq &x_{1}^{3} \leq x_{1}^{2}+x_{2}^{2}\\
x_{1}^{1}\leq &x_{1}^{3} \leq x_{1}^{1}+0.5x_{2}^{1}+0.25\\
\phantom{xxxxxxxxxx}x_{1}^{0}+x_{2}^{0}\leq &x_{1}^{3} \leq 1.5x_{1}^{0}+0.5x_{2}^{0}+0.25\\
0\leq &x_{1}^{3} \leq 1.25\\
\end{aligned}$ };


\coordinate (x8) at (H);
 \node at (x8) [above=2.6mm  of x8,blue] {[-0.5,1.5]};
\node at (x8) [below=5.5mm  of x8] {$\begin{aligned}
x_{2}^{3}\leq &x_{2}^{3} \leq x_{2}^{3}\\
x_{1}^{2} -x_{2}^{2}\leq &x_{2}^{3} \leq x_{1}^{2}-x_{2}^{2}\\
x_{1}^{1} -0.5x_{2}^{1}-0.25\leq &x_{2}^{3} \leq x_{1}^{1}\phantom{xxxxxxxxxxxxxx}\\
0.5x_{1}^{0}+1.5x_{2}^{0}-0.25\leq &x_{2}^{3} \leq x_{1}^{0}+x_{2}^{0}\\
-0.25\leq &x_{2}^{3} \leq 1\\
\end{aligned}$ };


\coordinate (x9) at (I);
 \node at (x9) [above=2.6mm  of x9,blue] {[0,1.5]};
 \node at (x9) [above=5.5mm  of x9,gray] { $x_{1}^{3}\leq x_{1}^{4} \leq x_{1}^{3}$ };
\coordinate (x10) at (J);
 \node at (x10) [above=2.6mm  of x10,blue] {[0,1.5]};
 \node at (x10) [below=5.5mm  of x10,gray] { $\phantom{xxxxxx}x_{2}^{3}\leq x_{2}^{4} \leq 0.8x_{2}^{3}+0.2$ };


\coordinate (x11) at (K);
\node at (x11) [above=2.6mm  of x11,blue] {[0,3]};

\coordinate (x12) at (L);
\node at (x12) [above=2.6mm  of x12,blue] {[0,1.5]};
\coordinate (x13) at (M);
\node at (x13) [above=6mm  of x13] { $\begin{aligned}
x_{1}^{6}\leq &x_{1}^{6} \leq x_{1}^{6}\\
x_{1}^{5}+1.2\leq &x_{1}^{6} \leq x_{1}^{5} + 1.2\\
x_{1}^{4} +x_{2}^{4}+1.2\leq &x_{1}^{6} \leq x_{1}^{4}+x_{2}^{4}+1.2\\
&\dots\\
1.2\leq &x_{1}^{6} \leq 3.25\\
\end{aligned}$};
\node at (x13) [above=2.6mm  of x13,blue] {[1.2,4.2]};

\coordinate (x14) at (N);
\node at (x14) [above=2.6mm  of x14,blue] {[0,1.5]};
\node at (x14) [below=5.5mm  of x14] { $\begin{aligned}
x_{2}^{6}\leq &x_{2}^{6} \leq x_{2}^{6}\\
x_{2}^{5}\leq &x_{2}^{6} \leq x_{2}^{5}\\
x_{2}^{4}\leq &x_{2}^{6} \leq x_{2}^{4}\\
&\dots\\
-0.25\leq &x_{1}^{6} \leq 1\\
\end{aligned}$ };



%\coordinate (H) at (E);
%\node at (H) [above=6mm  of H] { Hidden Layers };

 %\coordinate (OUT) at (K);
%\node at (OUT) [above=6mm  of OUT] { Output Layer };

\end{tikzpicture}
\caption{Robustness verification of a simple neural network with \hboxgpu and with \deeppoly.}
\label{Fi:nn}
\end{figure*}


==> neural_network_deeppoly.tex <==
\begin{figure*}[h!t]

\centering
\begin{tikzpicture}[font=\tiny\sffamily][scale=1]
    \node[shape=circle,draw=violet] (A) at (0,0) {$x_{1}^{1}$};
    \node[shape=circle,draw=violet] (B) at (0,-1.5) {$x_{2}^{1}$};
    \node[shape=circle,draw=gray] (C) at (2.7,0) {$x_{1}^{2}$};
    \node[shape=circle,draw=gray] (D) at (2.7,-1.5) {$x_{2}^{2}$};
    \node[shape=circle,draw=gray] (E) at (5.4,0) {$x_{1}^{3}$};
    \node[shape=circle,draw=gray] (F) at (5.4,-1.5) {$x_{2}^{3}$};
    \node[shape=circle,draw=gray] (G) at (8.1,0) {$x_{1}^{4}$} ;
    \node[shape=circle,draw=gray] (H) at (8.1,-1.5) {$x_{2}^{4}$} ;
     \node[shape=circle,draw=gray] (I) at (10.8,0) {$x_{1}^{5}$} ;
    \node[shape=circle,draw=gray] (J) at (10.8,-1.5) {$x_{2}^{5}$} ;
    \node[shape=circle,draw=purple] (K) at (13.5,0) {$x_{1}^{6}$} ;
    \node[shape=circle,draw=purple] (L) at (13.5,-1.5) {$x_{2}^{6}$} ;

    \path [->,blue] (A) edge node[left,above] {1} (C);
    \path [->,blue](B) edge node[left,below] {-1} (D);
    \path [->,blue](A) edge node[pos=0.25,left,above] {1} (D);
    \path [->,blue](B) edge node[pos=0.25,left,above] {1} (C);
    
    \path [->](C) edge node[left,above] {$max(0,x_{1}^{2})$} (E);
    \path [->](D) edge node[left,below] {$max(0,x_{2}^{2})$} (F);
    
    \path [->,blue] (E) edge node[left,above] {1} (G);
    \path [->,blue](F) edge node[left,below] {-1} (H);
    \path [->,blue](E) edge node[pos=0.25,left,above] {1} (H);
    \path [->,blue](F) edge node[pos=0.25,left,above] {1} (G);
    \path [->](G) edge node[left,above] {$max(0,x_{1}^{4})$} (I);
    \path [->](H) edge node[left,below] {$max(0,x_{2}^{4})$} (J);
    \path [->] (-1,0) edge node[left,above] {[0,0.5]} (A);
    \path [->](-1,-1.5) edge node[left,below] {[0,0.5]} (B);
    \path [->,blue] (I) edge node[left,above] {1} (K);
    \path [->,blue](J) edge node[pos=0.25,left,above] {1} (K);
    \path [->,blue] (I) edge node[pos=0.25,left,above] {0} (L);
    \path [->,blue](J) edge node[left,below] {1} (L);

    \coordinate (x1) at (A);
\node at (x1) [above=5.5mm  of x1] { $\begin{aligned} & \langle x_{1}^{1} \ge 0 ,\\
							&x_{1}^{1} \le 0.5,\\
							&l_{1}^{1}=0,
							u_{1}^{1}=0.5 \rangle \end{aligned}$ };




\coordinate (x2) at (B);
\node at (x2) [below=5.5mm  of x2] { $\begin{aligned}& \langle  x_{2}^{1} \ge 0,\\
							 &x_{2}^{1} \le 0.5,\\
							&l_{2}^{1}=0,
							u_{2}^{1}=0.5  \rangle \end{aligned}$ };


 \coordinate (x3) at (C);
\node at (x3) [above=5.5mm  of x3] { $\begin{aligned}&  \langle x_{1}^{2} \ge x_{1}^{1} +x_{2}^{1},\\
							 &x_{1}^{2} \le x_{1}^{1}+x_{2}^{1},\\
							&l_{1}^{2}=0,
							u_{1}^{2}=1 \rangle \end{aligned}$ };

\coordinate (x3) at (C);
\node at (x3) [above=2.6mm  of x3] {0};

\coordinate (x4) at (D);
\node at (x4) [below=5.5mm  of x4] { $\begin{aligned}& \langle x_{2}^{2} \ge x_{1}^{1} -x_{2}^{1},\\
							 &x_{2}^{2} \le x_{1}^{1}-x_{2}^{1},\\
							&l_{2}^{2}=-0.5,
							u_{2}^{2}=0.5 \rangle \end{aligned}$ };

\coordinate (x4) at (D);
\node at (x4) [below=2.6mm  of x4] {0};

\coordinate (x5) at (E);
\node at (x5) [above=5.5mm  of x5] { $\begin{aligned}&  \langle x_{1}^{3} \ge x_1^{2} ,\\
							 &x_{1}^{3}\le x_{1}^{2},\\
							&l_{1}^{3}=0,
							u_{1}^{3}=1 \rangle  \end{aligned}$ };

%\coordinate (x5) at (E);
%\node at (x5) [above=2.6mm  of x5] {0};

\coordinate (x6) at (F);
\node at (x6) [below=5.5mm  of x6] { $\begin{aligned}& \langle x_{2}^{3} \ge 0,\\
							&x_{2}^{3} \le 0.5 \cdot x_{2}^{2} + 0.25,\\
							&l_{2}^{3}=0,
							u_{2}^{3}=0.5 \rangle \end{aligned}$ };

%\coordinate (x6) at (F);
%\node at (x6) [above=2.6mm  of x6] {0};

\coordinate (x7) at (G);
\node at (x7) [above=5.5mm  of x7] { $\begin{aligned}& \langle x_{1}^{4} \ge x_{1}^{3} +x_{2}^{3},\\
							 &x_{1}^{4} \le x_{1}^{3}+x_{2}^{3},\\
							&l_{1}^{4}=0,
							u_{1}^{4}=1.25 \rangle \end{aligned}$ };

\coordinate (x7) at (G);
\node at (x7) [above=2.6mm  of x7] {0};

\coordinate (x8) at (H);
\node at (x8) [below=5.5mm  of x8] { $\begin{aligned}& \langle  x_{2}^{4} \ge x_{1}^{3} -x_{2}^{3},\\
							& x_{2}^{4} \le x_{1}^{3}-x_{2}^{3},\\
							&l_{2}^{4}=-0.25,
							u_{2}^{4}=1 \rangle \end{aligned}$ };

\coordinate (x8) at (H);
\node at (x8) [below=2.6mm  of x8] {0};

\coordinate (x9) at (I);
\node at (x9) [above=6mm  of x9] { $\begin{aligned}&  \langle x_{1}^{5} \ge x_{1}^{4} ,\\
							& x_{1}^{5}\le x_{1}^{4},\\
							&l_{1}^{5}=0,
							u_{1}^{5}=1.25 \rangle \end{aligned}$ };

%\coordinate (x9) at (H);
%\node at (x9) [above=2.6mm  of x9] {0};

\coordinate (x10) at (J);
\node at (x10) [below=5.5mm  of x10] { $\begin{aligned}& \langle x_{2}^{5} \ge x_2^{4},\\
							&x_{2}^{5} \le 0.8 \cdot x_{2}^{4} + 0.2,\\
							&l_{2}^{5}=-0.25,
							u_{2}^{5}=1 \rangle \end{aligned}$ };
%\coordinate (x10) at (K);
%\node at (x10) [above=2.6mm  of x10] {0};


\coordinate (x11) at (K);
\node at (x11) [above=6mm  of x11] { $\begin{aligned}& \langle x_{1}^{6} \ge x_{1}^{5}+x_{2}^{5}+1,\\
							&x_{1}^{6} \le x_{1}^{5} + x_{2}^{5}+1,\\
							&l_{1}^{6}=1,
							u_{1}^{6}=3.05 \rangle \end{aligned}$ };
\coordinate (x11) at (K);
\node at (x11) [above=2.6mm  of x11] {1};

\coordinate (x12) at (L);
\node at (x12) [below=5.5mm  of x12] { $\begin{aligned}& \langle x_{2}^{6} \ge x_{2}^{5},\\
							&x_{2}^{6} \le x_{2}^{5},\\
							&l_{2}^{6}=-0.25,
							u_{2}^{6}=1 \rangle \end{aligned}$ };

\coordinate (x12) at (L);
\node at (x12) [below=2.6mm  of x12] {0};

%\coordinate (H) at (E);
%\node at (H) [above=6mm  of H] { Hidden Layers };

 %\coordinate (OUT) at (K);
%\node at (OUT) [above=6mm  of OUT] { Output Layer };

\end{tikzpicture}
\caption{Robustness verification of a simple fully connected network with \deeppoly.}
\label{Fi:nn}
\end{figure*}


==> relu.tex <==
\begin{figure*}
%\centering

\begin{tikzpicture}
\coordinate (l1) at (-2,0);
\coordinate (u1) at (2,2);
\coordinate (v1) at (2,0);
\coordinate (o1) at (0,0);
\coordinate (startx1) at (-2.3,0);
\coordinate (endx1) at (2.5,0);
\coordinate (starty1) at (0,-2);
\coordinate (endy1) at (0,2.6);
\coordinate (startl1) at (-2,-2);
\coordinate (endl1) at (-2,2);
\coordinate (startu1) at (2,-2);
\coordinate (endu1) at (2,2);

\def\distx{6}
\def\disty{4}
\def\height{-0.9}
\def\width{1.1}

\coordinate (l2) at ($(l1) + (\distx,0)$);
\coordinate (u2) at ($(u1) + (\distx,0)$);
\coordinate (v2) at ($(startl1) + (\distx,0)$);
\coordinate (o2) at ($(0,0) + (\distx,0)$);
\coordinate (startx2) at ($(startx1) + (\distx,0)$);
\coordinate (endx2) at ($(endx1) + (\distx,0)$);
\coordinate (starty2) at ($(starty1)+(\distx,0)$);
\coordinate (endy2) at ($(endy1) + (\distx,0)$);
\coordinate (startl2) at ($(startl1) + (\distx,0)$);
\coordinate (endl2) at ($(endl1) + (\distx,0)$);
\coordinate (startu2) at ($(startu1) + (\distx,0)$);
\coordinate (endu2) at ($(endu1) + (\distx,0)$);

\coordinate (l3) at ($(l1) + (-\distx,0)$);
\coordinate (u3) at ($(u1) + (-\distx,0)$);
\coordinate (v3) at ($(0,0) + (-\distx,0)$);
\coordinate (startx3) at ($(startx1) + (-\distx,0)$);
\coordinate (endx3) at ($(endx1) + (-\distx,0)$);
\coordinate (starty3) at ($(starty1)+(-\distx,0)$);
\coordinate (endy3) at ($(endy1) + (-\distx,0)$);
\coordinate (startl3) at ($(startl1) + (-\distx,0)$);
\coordinate (endl3) at ($(endl1) + (-\distx,0)$);
\coordinate (startu3) at ($(startu1) + (-\distx,0)$);
\coordinate (endu3) at ($(endu1) + (-\distx,0)$);

\coordinate (l4) at ($(l1) + (\distx,\disty)$);
\coordinate (u4) at ($(u1) + (\distx,\disty)$);
\coordinate (v4) at ($(1,0.5) + (\distx,\disty)$);
\coordinate (w4) at ($(-1,-0.5) + (\distx,\disty)$);
\coordinate (o4) at ($(0,0) + (\distx,\disty)$);
\coordinate (startx4) at ($(startx1) + (\distx,\disty)$);
\coordinate (endx4) at ($(endx1) + (\distx,\disty)$);
\coordinate (starty4) at ($(starty1)+(\distx,\disty)$);
\coordinate (endy4) at ($(endy1) + (\distx,\disty)$);
\coordinate (startl4) at ($(startl1) + (\distx,\disty)$);
\coordinate (endl4) at ($(endl1) + (\distx,\disty)$);
\coordinate (startu4) at ($(startu1) + (\distx,\disty)$);
\coordinate (endu4) at ($(endu1) + (\distx,\disty)$);

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\draw[->] (startx1) --(endx1);
\draw[->] (starty1)  --(endy1);
\draw (l1)[thick] --(u1);
\draw (l1)[thick] --(v1);
%\draw (o1)[thick,teal,dashed] --(u1);
\draw (startl1) --(endl1);
\draw (startu1) --(endu1);

\draw[fill=lightgray]  (l1) -- (v1) -- (u1) -- cycle;

\coordinate (X1) at (endx1);
\node at (X1) [right=0.1mm  of X1] { $x^{\layerno}_i$};

\coordinate (Y1) at (endy1);
\node at (Y1) [above=0.1mm  of Y1] { $x^{\layerno+1}_i$};

%\draw (1,-0.1) --(1,0.1);

\coordinate (P1) at ($0.4*(endu1) + 0.6*(startu1)$);
\node at (P1) [right=0.1mm  of P1] { $u$};

\coordinate (R1) at ($0.4*(endl1) + 0.6*(startl1)$);
\node at (R1) [left=0.1mm  of R1] { $l$};

\coordinate (Q1) at ($(endy1)+(-1.96,-2)$);
\node at (Q1) [right=0.1mm  of Q1, rotate=26] { $\lambda \cdot x_{i} + \mu$};

\coordinate (O1) at (starty1);
\node at (O1) [below=0.1mm  of O1] {  (b) };

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\draw[->] (startx2) --(endx2);
\draw[->] (starty2) --(endy2);
\draw (l2)[thick] --(u2);
\draw (u2)[thick] --(v2);
%\draw (l2)[thick,teal,dashed] --(o2);
\draw (startl2)  --(endl2);
\draw (startu2) --(endu2);

\draw[fill=lightgray]  (l2) -- (v2) -- (u2) -- cycle;

\coordinate (X2) at (endx2);
\node at (X2) [right=0.1mm  of X2] { $x^{\layerno}_i$};

\coordinate (Y2) at (endy2);
\node at (Y2) [above=0.1mm  of Y2] { $x^{\layerno+1}_i$};

\coordinate (P2) at ($0.4*(endu2) + 0.6*(startu2)$);
\node at (P2) [right=0.1mm  of P2] { $u$};

\coordinate (R2) at ($0.4*(endl2) + 0.6*(startl2)$);
\node at (R2) [left=0.1mm  of R2] { $l$};

\coordinate (Q2) at ($(endy2)+(-1.96,-2)$);
\node at (Q2) [right=0.1mm  of Q2, rotate=26] { $\lambda \cdot x^{\layerno}_i + \mu$};


\coordinate (S2) at ($(v2)+(0.4,0)$);
\node at (S2) [right=0.1mm  of S2, rotate=45] { $x^{\layerno}_i$};

\coordinate (O2) at (starty2);
\node at (O2) [below=0.1mm  of O2] {  (c) };

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\draw[->] (startx3) --(endx3);
\draw[->] (starty3) --(endy3);
\draw (l3)[thick] --(u3);
\draw (u3)[thick] --(v3);
\draw (l3)[thick] --(v3);
\draw (startl3)  --(endl3);
\draw (startu3) --(endu3);

\draw[fill=lightgray]  (l3) -- (v3) -- (u3) -- cycle;

\coordinate (X3) at (endx3);
\node at (X3) [right=0.1mm  of X3] { $x^{\layerno}_i$};

\coordinate (Y3) at (endy3);
\node at (Y3) [above=0.1mm  of Y3] { $x^{\layerno+1}_i$};

\coordinate (P3) at ($0.4*(endu3) + 0.6*(startu3)$);
\node at (P3) [right=0.1mm  of P3] { $u$};

\coordinate (R3) at ($0.4*(endl3) + 0.6*(startl3)$);
\node at (R3) [left=0.1mm  of R3] { $l$};

\coordinate (Q3) at ($(endy3)+(-1.96,-2)$);
\node at (Q3) [right=0.1mm  of Q3, rotate=26] { $\lambda \cdot x^{\layerno}_i + \mu$};


\coordinate (S3) at ($(v3)+(0.4,-0.05)$);
\node at (S3) [right=0.1mm  of S3,rotate=45] { $x^{\layerno}_i$};
\coordinate (O3) at (starty3);
\node at (O3) [below=0.1mm  of O3] {  (a) };


\end{tikzpicture}
\vspace*{-3mm}
\caption{Convex approximations for the ReLU function: (a) shows the convex approximation \cite{Ehlers:17} with the minimum area in the input-output plane, (b) and (c) show the two convex approximations used in \deeppoly. In the figure, $\lambda= u/(u-l)$ and $\mu=-l\cdot u/(u-l)$.}
\label{Fi:relu}
\end{figure*}
